Generative Adversarial Neural Architecture Search

Despite the empirical success of neural architecture search (NAS) in deep learning applications, the optimality, reproducibility and cost of NAS schemes remain hard to assess. In this paper, we propose Generative Adversarial NAS (GA-NAS) with theoretically provable convergence guarantees, promoting stability and reproducibility in neural architecture search. Inspired by importance sampling, GA-NAS iteratively fits a generator to previously discovered top architectures, thus increasingly focusing on important parts of a large search space. Furthermore, we propose an efficient adversarial learning approach, where the generator is trained by reinforcement learning based on rewards provided by a discriminator, thus being able to explore the search space without evaluating a large number of architectures. Extensive experiments show that GA-NAS beats the best published results under several cases on three public NAS benchmarks. In the meantime, GA-NAS can handle ad-hoc search constraints and search spaces. We show that GA-NAS can be used to improve already optimized baselines found by other NAS methods, including EfficientNet and ProxylessNAS, in terms of ImageNet accuracy or the number of parameters, in their original search space.

==> impact.tex <==
\section*{Broader Impact}

This paper introduces Generative Adversarial NAS (GA-NAS) as a new method to neural architecture search.

Although our experimental results are only reported for the best neural architecture network for image classification tasks, our algorithm is a general NAS algorithm and can be applied to diverse range of applications. By incorporating the corresponding search spaces to our search algorithm, we can find appropriate neural architectures for the object detection and image segmentation as well as Neural Language Processing (NLP) tasks.

GA-NAS performs search on the micro-level, where the best cell architectures are discovered. These cells can then be taken and used in macro-level experiments, where the candidate cells are fixed. Macro search pertains to how fixed cells are ordered within a larger network. The advantages are further emphasized by how GA-NAS can handle constrained search objectives. GA-NAS accomplishes this by mimicking and improving example ground-truth models. The combined effects of these benefits is that GA-NAS can be integrated as part of a larger system that not only generates highly complex models, but gradually improves upon their performance. These concepts are extremely important to AutoML and NAS for industrial purposes.

% 3) Promoted reproducibility and benchmarking among NAS algorithms, by comparing lots of algorithms on two bechmarking datasets nb101 nb201. Eliminited doubts about reproduciblity and sensitivity to random seeds. 
By experimenting on two publicly available NAS benchmarks, i.e., NAS-Bench-101 and 201, we have ensured a fair comparison on the performance and generalizability of popular NAS algorithms. 
Previous studies have indicated that re-producibility is a often a concern for NAS algorithms because each algorithm has its own search space, performance metrics and evaluation methods.
In comparison, our work eliminated doubts about re-producibility, and by conducting multiple runs under different random seeds, we also significantly reduced the sensitivity to random initializations.

% 4) Saves searching cost and carbon footprint of NAS. NAS initially takes hundreds of GPU days
Originally, NAS is a resource-intensive task. In real-world applications, where accuracy of each architecture is not available, it would potentially take thousands of GPU hours to fully evaluate every candidate architecture in order to locate the best one. 
In comparison, our algorithm is evaluated on publicly available benchmarks, which not only improves comparability to other approaches, but also significantly lowers the cost and the carbon footprint of running NAS experiments.
Even in a real-world application, GA-NAS is compatible with many resource-efficient evaluation methods, such as using a weight-sharing supernet or a performance prediction model, so a user would have complete freedom in choosing the most cost-effective and environmentally friendly evaluation method that fits his/her problem setting. 

Another key aspect of GA-NAS that contributes to its superior resource efficiency is the sampling efficiency during search.
Specifically, on NAS-Bench-101 we are able to locate the 3rd most accurate cell among 423,624 cells with 533 evaluations, and the 2nd most accurate with 1606 evaluations, on average.
This indicates that GA-NAS often evaluates less number of cells to find the best performing cell, compared to other approaches.
In a real-world application, less number of evaluations translates into energy and cost savings. Therefore, further reducing the overall carbon footprint.

By experimenting under a constrained objective that takes both accuracy and speed into consideration,
GA-NAS also has a positive impact on applications with limited resources. 
Finding an architecture with high accuracy and small model size positively affects the deploy-ability of a model on resource-limited devices and decreasing the energy consumption of these devices. 
The search algorithm will improve the search for architectures tailored to a specific task given certain constraints.


% We are aware that in real scenarios, where such a benchmark is not available, the task will be resource consuming and requires more experimentation. Still, this might incur the consumption of more GPU resources for tasks, where datasets are not available. 
% We believe that the focus on the search algorithm within limited data can overcome these issues.
